Spatial and Temporal Evaluations of the Liquid Argon Purity in ProtoDUNE-SP

Liquid argon time projection chambers (LArTPCs) rely on highly pure argon to ensure that ionization electrons produced by charged particles reach readout arrays. ProtoDUNE Single-Phase (ProtoDUNE-SP) was an approximately 700-ton liquid argon detector intended to prototype the Deep Underground Neutrino Experiment (DUNE) Far Detector Horizontal Drift module. It contains two drift volumes bisected by the cathode plane assembly, which is biased to create an almost uniform electric field in both volumes. The DUNE Far Detector modules must have robust cryogenic systems capable of filtering argon and supplying the TPC with clean liquid. This paper will explore comparisons of the argon purity measured by the purity monitors with those measured using muons in the TPC from October 2018 to November 2018. A new method is introduced to measure the liquid argon purity in the TPC using muons crossing both drift volumes of ProtoDUNE-SP. For extended periods on the timescale of weeks, the drift electron lifetime was measured to be above 30 ms using both systems. A particular focus will be placed on the measured purity of argon as a function of position in the detector.

==> export_xml_authors_2025-05-05_arxiv.tex <==
# Plain-text author list (see https://arxiv.org/help/prep) produced at 2025-05-05, from master list generated at 2025-05-05
DUNE Collaboration: S. Abbaslu, A. Abed Abud, R. Acciarri, L. P. Accorsi, M. A. Acero, M. R. Adames, G. Adamov, M. Adamowski, C. Adriano, F. Akbar, F. Alemanno, N. S. Alex, K. Allison, M. Alrashed, A. Alton, R. Alvarez, T. Alves, A. Aman, H. Amar, P. Amedo, J. Anderson, D. A. ~Andrade, C. Andreopoulos, M. Andreotti, M. P. Andrews, F. Andrianala, S. Andringa, F. Anjarazafy, S. Ansarifard, D. Antic, M. Antoniassi, A. Aranda-Fernandez, L. Arellano, E. Arrieta Diaz, M. A. Arroyave, M. Arteropons, J. Asaadi, M. Ascencio, A. Ashkenazi, D. Asner, L. Asquith, E. Atkin, D. Auguste, A. Aurisano, V. Aushev, D. Autiero, D. \'Avila G{\'o}mez, M. B. Azam, F. Azfar, A. Back, J. J. Back, Y. Bae, I. Bagaturia, L. Bagby, D. Baigarashev, S. Balasubramanian, A. Balboni, P. Baldi, W. Baldini, J. Baldonedo, B. Baller, B. Bambah, F. Barao, D. Barbu, G. Barenboim, P.\ Barham~Alz\'as, G. J. Barker, W. Barkhouse, G. Barr, A. Barros, N. Barros, D. Barrow, J. L. Barrow, A. Basharina-Freshville, A. Bashyal, V. Basque, M. Bassani, D. Basu, C. Batchelor, L. Bathe-Peters, J.B.R. Battat, F. Battisti, J. Bautista, F. Bay, J. L. L. Bazo Alba, J. F. Beacom, E. Bechetoille, B. Behera, E. Belchior, B. Bell, G. Bell, L. Bellantoni, G. Bellettini, V. Bellini, O. Beltramello, A. Belyaev, C. Benitez Montiel, D. Benjamin, F. Bento Neves, J. Berger, S. Berkman, J. Bermudez, J. Bernal, P. Bernardini, A. Bersani, E. Bertholet, E. Bertolini, S. Bertolucci, M. Betancourt, A. Betancur Rodr\'iguez, Y. Bezawada, A. T. Bezerra, A. Bhat, V. Bhatnagar, J. Bhatt, M. Bhattacharjee, S. Bhattacharjee, M. Bhattacharya, S. Bhuller, B. Bhuyan, S. Biagi, J. Bian, K. Biery, B. Bilki, M. Bishai, A. Blake, F. D. Blaszczyk, G. C. Blazey, E. Blucher, B. Bogart, J. Boissevain, S. Bolognesi, T. Bolton, L. Bomben, M. Bonesini, C. Bonilla-Diaz, A. Booth, F. Boran, R. Borges Merlo, N. Bostan, G. Botogoske, B. Bottino, R. Bouet, J. Boza, J. Bracinik, B. Brahma, D. Brailsford, F. Bramati, A. Branca, A. Brandt, J. Bremer, S. J. Brice, V. Brio, C. Brizzolari, C. Bromberg, J. Brooke, A. Bross, G. Brunetti, M. B. Brunetti, N. Buchanan, H. Budd, J. Buergi, A. Bundock, D. Burgardt, S. Butchart, G. Caceres V., R. Calabrese, R. Calabrese, J. Calcutt, L. Calivers, E. Calvo, A. Caminata, A. F. Camino, W. Campanelli, A. Campani, A. Campos Benitez, N. Canci, J. Cap{\'o}, I. Caracas, D. Caratelli, D. Carber, J. M. Carceller, G. Carini, B. Carlus, M. F. Carneiro, P. Carniti, I. Caro Terrazas, H. Carranza, N. Carrara, L. Carroll, T. Carroll, A. Carter, E. Casarejos, D. Casazza, J. F. Casta{\~n}o Forero, F. A. Casta{\~n}o, C. Castromonte, E. Catano-Mur, C. Cattadori, F. Cavalier, F. Cavanna, S. Centro, G. Cerati, C. Cerna, A. Cervelli, A. Cervera Villanueva, J. Chakrani, M. Chalifour, A. Chappell, A. Chatterjee, B. Chauhan, C. Chavez Barajas, H. Chen, M. Chen, W. C. Chen, Y. Chen, Z. Chen, D. Cherdack, S. S. Chhibra, C. Chi, F. Chiapponi, R. Chirco, N. Chitirasreemadam, K. Cho, S. Choate, G. Choi, D. Chokheli, P. S. Chong, B. Chowdhury, D. Christian, M. Chung, E. Church, M. F. Cicala, M. Cicerchia, V. Cicero, R. Ciolini, P. Clarke, G. Cline, A. G. Cocco, J. A. B. Coelho, A. Cohen, J. Collazo, J. Collot, H. Combs, J. M. Conrad, L. Conti, T. Contreras, M. Convery, K. Conway, S. Copello, P. Cova, C. Cox, L. Cremonesi, J. I. Crespo-Anad\'on, M. Crisler, E. Cristaldo, J. Crnkovic, G. Crone, R. Cross, A. Cudd, C. Cuesta, Y. Cui, F. Curciarello, D. Cussans, J. Dai, O. Dalager, W. Dallaway, R. D'Amico, H. da Motta, Z. A. Dar, R. Darby, L. Da Silva Peres, Q. David, G. S. Davies, S. Davini, J. Dawson, R. De Aguiar, P. Debbins, M. P. Decowski, A. de Gouv\^ea, P. C. De Holanda, P. De Jong, P. Del Amo Sanchez, G. De Lauretis, A. Delbart, M. Delgado, A. Dell'Acqua, G. Delle Monache, N. Delmonte, P. De Lurgio, G. De Matteis, J. R. T. de Mello Neto, A. P. A. De Mendonca, D. M. DeMuth, S. Dennis, C. Densham, P. Denton, G. W. Deptuch, A. De Roeck, V. De Romeri, J. P. Detje, J. Devine, K. Dhanmeher, R. Dharmapalan, M. Dias, A. Diaz, J. S. D\'iaz, F. D{\'\i}az, F. Di Capua, A. Di Domenico, S. Di Domizio, S. Di Falco, L. Di Giulio, P. Ding, L. Di Noto, E. Diociaiuti, G. Di Sciascio, V. Di Silvestre, C. Distefano, R. Di Stefano, R. Diurba, M. Diwan, Z. Djurcic, S. Dolan, M. Dolce, M. J. Dolinski, D. Domenici, S. Dominguez, S. Donati, S. Doran, D. Douglas, T.A. Doyle, F. Drielsma, D. Duchesneau, K. Duffy, K. Dugas, P. Dunne, B. Dutta, D. A. Dwyer, A. S. Dyshkant, S. Dytman, M. Eads, A. Earle, S. Edayath, D. Edmunds, J. Eisch, W. Emark, P. Englezos, A. Ereditato, T. Erjavec, C. O. Escobar, J. J. Evans, E. Ewart, A. C. Ezeribe, K. Fahey, A. Falcone, M. Fani', D. Faragher, C. Farnese, Y. Farzan, J. Felix, Y. Feng, M. Ferreira da Silva, G. Ferry, E. Fialova, L. Fields, P. Filip, A. Filkins, F. Filthaut, G. Fiorillo, M. Fiorini, S. Fogarty, W. Foreman, J. Fowler, J. Franc, K. Francis, D. Franco, J. Freeman, J. Fried, A. Friedland, M. Fucci, S. Fuess, I. K. Furic, K. Furman, A. P. Furmanski, R. Gaba, A. Gabrielli, A. M~Gago, F. Galizzi, H. Gallagher, M. Galli, N. Gallice, V. Galymov, E. Gamberini, T. Gamble, R. Gandhi, S. Ganguly, F. Gao, S. Gao, D. Garcia-Gamez, M. \'A. Garc\'ia-Peris, F. Gardim, S. Gardiner, A. Gartman, A. Gauch, P. Gauzzi, S. Gazzana, G. Ge, N. Geffroy, B. Gelli, S. Gent, L. Gerlach, A. Ghosh, T. Giammaria, D. Gibin, I. Gil-Botella, A. Gioiosa, S. Giovannella, A. K. Giri, V. Giusti, D. Gnani, O. Gogota, S. Gollapinni, K. Gollwitzer, R. A. Gomes, L. S. Gomez Fajardo, D. Gonzalez-Diaz, J. Gonzalez-Santome, M. C. Goodman, S. Goswami, C. Gotti, J. Goudeau, C. Grace, E. Gramellini, R. Gran, P. Granger, C. Grant, D. R. Gratieri, G. Grauso, P. Green, S. Greenberg, W. C. Griffith, K. Grzelak, L. Gu, W. Gu, V. Guarino, M. Guarise, R. Guenette, M. Guerzoni, D. Guffanti, A. Guglielmi, F. Y. Guo, A. Gupta, V. Gupta, G. Gurung, D. Gutierrez, P. Guzowski, M. M. Guzzo, S. Gwon, A. Habig, L. Haegel, R. Hafeji, L. Hagaman, A. Hahn, J. Hakenm\"uller, T. Hamernik, P. Hamilton, J. Hancock, M. Handley, F. Happacher, B. Harris, D. A. Harris, L. Harris, A. L. Hart, J. Hartnell, T. Hartnett, J. Harton, T. Hasegawa, C. M. Hasnip, R. Hatcher, S. Hawkins, J. Hays, M. He, A. Heavey, K. M. Heeger, A. Heindel, J. Heise, P. Hellmuth, L. Henderson, K. Herner, V. Hewes, A. Higuera, A. Himmel, E. Hinkle, L.R. Hirsch, J. Ho, J. Hoefken Zink, J. Hoff, A. Holin, T. Holvey, C. Hong, S. Horiuchi, G. A. Horton-Smith, R. Hosokawa, T. Houdy, B. Howard, R. Howell, I. Hristova, M. S. Hronek, H. Hua, J. Huang, R.G. Huang, X. Huang, Z. Hulcher, A. Hussain, G. Iles, N. Ilic, A. M. Iliescu, R. Illingworth, G. Ingratta, A. Ioannisian, M. Ismerio Oliveira, C.M. Jackson, V. Jain, E. James, W. Jang, B. Jargowsky, D. Jena, I. Jentz, C. Jiang, J. Jiang, A. Jipa, J. H. Jo, F. R. Joaquim, W. Johnson, C. Jollet, R. Jones, N. Jovancevic, M. Judah, C. K. Jung, K. Y. Jung, T. Junk, Y. Jwa, M. Kabirnezhad, A. C. Kaboth, I. Kadenko, O. Kalikulov, D. Kalra, M. Kandemir, S. Kar, G. Karagiorgi, G. Karaman, A. Karcher, Y. Karyotakis, S. P. Kasetti, L. Kashur, A. Kauther, N. Kazaryan, L. Ke, E. Kearns, P.T. Keener, K.J. Kelly, R. Keloth, E. Kemp, O. Kemularia, Y. Kermaidic, W. Ketchum, S. H. Kettell, N. Khan, A. Khvedelidze, D. Kim, J. Kim, M. J. Kim, S. Kim, B. King, M. King, M. Kirby, A. Kish, J. Klein, J. Kleykamp, A. Klustova, T. Kobilarcik, L. Koch, K. Koehler, L. W. Koerner, D. H. Koh, M. Kordosky, T. Kosc, V. A. Kosteleck\'y, I. Kotler, M. Kovalcuk, W. Krah, R. Kralik, M. Kramer, F. Krennrich, T. Kroupova, S. Kubota, M. Kubu, V. A. Kudryavtsev, G. Kufatty, S. Kuhlmann, A. Kumar, J. Kumar, M. Kumar, P. Kumar, P. Kumar, S. Kumaran, J. Kunzmann, V. Kus, T. Kutter, J. Kvasnicka, T. Labree, M. Lachat, T. Lackey, I. Lal{\u{a}}u, A. Lambert, B. J. Land, C. E. Lane, N. Lane, K. Lang, T. Langford, M. Langstaff, F. Lanni, J. Larkin, P. Lasorak, D. Last, A. Laundrie, G. Laurenti, E. Lavaut, H. Lay, I. Lazanu, R. LaZur, M. Lazzaroni, S. Leardini, J. Learned, T. LeCompte, G. Lehmann Miotto, R. Lehnert, M. Leitner, H. Lemoine, D. Leon Silverio, L. M. Lepin, J.-Y~Li, S. W. Li, Y. Li, R. Lima, C. S. Lin, D. Lindebaum, S. Linden, R. A. Lineros, A. Lister, B. R. Littlejohn, J. Liu, Y. Liu, S. Lockwitz, I. Lomidze, K. Long, J.Lopez, I. L{\'o}pez de Rego, N. L{\'o}pez-March, J. M. LoSecco, A. Lozano Sanchez, X.-G. Lu, K.B. Luk, X. Luo, E. Luppi, A. A. Machado, P. Machado, C. T. Macias, J. R. Macier, M. MacMahon, S. Magill, C. Magueur, K. Mahn, A. Maio, N. Majeed, A. Major, K. Majumdar, A. Malige, S. Mameli, M. Man, R. C. Mandujano, J. Maneira, S. Manly, K. Manolopoulos, M. Manrique Plata, S. Manthey Corchado, L. Manzanillas-Velez, E. Mao, M. Marchan, A. Marchionni, D. Marfatia, C. Mariani, J. Maricic, F. Marinho, A. D. Marino, T. Markiewicz, F. Das Chagas Marques, M. Marshak, C. M. Marshall, J. Marshall, L. Martina, J. Mart{\'\i}n-Albo, D.A. Martinez Caicedo , M. Martinez-Casales, F. Mart{\'i}nez L{\'o}pez, S. Martynenko, V. Mascagna, A. Mastbaum, M. Masud, F. Matichard, G. Matteucci, J. Matthews, C. Mauger, N. Mauri, K. Mavrokoridis, I. Mawby, F. Mayhew, T. McAskill, N. McConkey, B. McConnell, K. S. McFarland, C. McGivern, C. McGrew, A. McNab, C. McNulty, J. Mead, L. Meazza, V. C. N. Meddage, A. Medhi, M. Mehmood, B. Mehta, P. Mehta, F. Mei, P. Melas, L. Mellet, T. C. D. Melo, O. Mena, H. Mendez, D. P. M{\'e}ndez, A. Menegolli, G. Meng, A. C. E. A. Mercuri, A. Meregaglia, M. D. Messier, S. Metallo, W. Metcalf, M. Mewes, H. Meyer, T. Miao, J. Micallef, A. Miccoli, G. Michna, R. Milincic, F. Miller, G. Miller, W. Miller, A. Minotti, L. Miralles Verge, C. Mironov, S. Miscetti, C. S. Mishra, P. Mishra, S. R. Mishra, D. Mladenov, I. Mocioiu, A. Mogan, R. Mohanta, T. A. Mohayai, N. Mokhov, J. Molina, L. Molina Bueno, E. Montagna, A. Montanari, C. Montanari, D. Montanari, D. Montanino, L. M. Monta{\~n}o Zetina, M. Mooney, A. F. Moor, M. Moore, Z. Moore, D. Moreno, G. Moreno-Granados, O. Moreno-Palacios, L. Morescalchi, C. Morris, E. Motuk, C. A. Moura, G. Mouster, W. Mu, L. Mualem, J. Mueller, M. Muether, F. Muheim, A. Muir, Y. Mukhamejanov, A. Mukhamejanova, M. Mulhearn, D. Munford, L. J. Munteanu, H. Muramatsu, J. Muraz, M. Murphy, T. Murphy, A. Mytilinaki, J. Nachtman, Y. Nagai, S. Nagu, D. Naples, S. Narita, J. Nava, A. Navrer-Agasson, N. Nayak, M. Nebot-Guinot, A. Nehm, J. K. Nelson, O. Neogi, J. Nesbit, M. Nessi, D. Newbold, M. Newcomer, D. Newmark, R. Nichol, F. Nicolas-Arnaldos, A. Nielsen, A. Nikolica, J. Nikolov, E. Niner, X. Ning, K. Nishimura, A. Norman, A. Norrick, P. Novella, A. Nowak, J. A. Nowak, M. Oberling, J. P. Ochoa-Ricoux, S. Oh, S.B. Oh, A. Olivier, T. Olson, Y. Onel, Y. Onishchuk, A. Oranday, M. Osbiston, J. A. Osorio V{\'e}lez, L. O'Sullivan, L. Otiniano Ormachea, L. Pagani, G. Palacio, O. Palamara, S. Palestini, J. M. Paley, M. Pallavicini, C. Palomares, S. Pan, M. Panareo, P. Panda, V. Pandey, W. Panduro Vazquez, E. Pantic, V. Paolone, A. Papadopoulou, R. Papaleo, D. Papoulias, S. Paramesvaran, J. Park, S. Parke, S. Parsa, S. Parveen, M. Parvu, D. Pasciuto, S. Pascoli, L. Pasqualini, J. Pasternak, G. Patel, J. L. Paton, C. Patrick, L. Patrizii, R. B. Patterson, T. Patzak, A. Paudel, J. Paul, L. Paulucci, Z. Pavlovic, G. Pawloski, D. Payne, A. Peake, V. Pec, E. Pedreschi, S. J. M. Peeters, W. Pellico, E. Pennacchio, A. Penzo, O. L. G. Peres, L. P{\'e}rez-Molina, C. Pernas, J. Perry, D. Pershey, G. Pessina, G. Petrillo, C. Petta, R. Petti, M. Pfaff, V. Pia, G. M. Piacentino, L. Pickering, L. Pierini, F. Pietropaolo, V.L.Pimentel, G. Pinaroli, S. Pincha, J. Pinchault, K. Pitts, P. Plesniak, K. Pletcher, K. Plows, C. Pollack, T. Pollmann, F. Pompa, X. Pons, N. Poonthottathil, V. Popov, F. Poppi, J. Porter, L. G. Porto Paix{\~a}o, M. Potekhin, M. Pozzato, R. Pradhan, T. Prakash, M. Prest, F. Psihas, D. Pugnere, D. Pullia, X. Qian, J. Queen, J. L. Raaf, M. Rabelhofer, V. Radeka, J. Rademacker, F. Raffaelli, A. Rafique, A. Rahe, S. Rajagopalan, M. Rajaoalisoa, I. Rakhno, L. Rakotondravohitra, M. A. Ralaikoto, L. Ralte, M. A. Ramirez Delgado, B. Ramson, S. S. Randriamanampisoa, A. Rappoldi, G. Raselli, T. Rath, P. Ratoff, R. Ray, H. Razafinime, R. F. Razakamiandra, E. M. Rea, J. S. Real, B. Rebel, R. Rechenmacher, J. Reichenbacher, S. D. Reitzner, E. Renner, S. Repetto, S. Rescia, F. Resnati, C. Reynolds, M. Ribas, S. Riboldi, C. Riccio, G. Riccobene, J. S. Ricol, M. Rigan, A. Rikalo, E. V. Rinc{\'o}n, A. Ritchie-Yates, D. Rivera, A. Robert, A. Roberts, E. Robles, M. Roda, D. Rodas Rodr{\'\i}guez, M. J. O. Rodrigues, J. Rodriguez Rondon, S. Rosauro-Alcaraz, P. Rosier, D. Ross, M. Rossella, M. Ross-Lonergan, T. Rotsy, N. Roy, P. Roy, P. Roy, C. Rubbia, D. Rudik, A. Ruggeri, G. Ruiz Ferreira, K. Rushiya, B. Russell, S. Sacerdoti, N. Saduyev, S. K. Sahoo, N. Sahu, S. Sakhiyev, P. Sala, G. Salmoria, S. Samanta, M. C. Sanchez, A. S{\'a}nchez-Castillo, P. Sanchez-Lucas, D. A. Sanders, S. Sanfilippo, D. Santoro, N. Saoulidou, P. Sapienza, I. Sarcevic, I. Sarra, G. Savage, V. Savinov, G. Scanavini, A. Scanu, A. Scaramelli, T. Schefke, H. Schellman, S. Schifano, P. Schlabach, D. Schmitz, A. W. Schneider, K. Scholberg, A. Schroeder, A. Schukraft, B. Schuld, S. Schwartz, A. Segade, E. Segreto, A. Selyunin, C. R. Senise, J. Sensenig, S.H. Seo, D. Seppela, M. H. Shaevitz, P. Shanahan, P. Sharma, R. Kumar, S. Sharma Poudel, K. Shaw, T. Shaw, K. Shchablo, J. Shen, C. Shepherd-Themistocleous, J. Shi, W. Shi, S. Shin, S. Shivakoti, A. Shmakov, I. Shoemaker, D. Shooltz, R. Shrock, M. Siden, J. Silber, L. Simard, J. Sinclair, G. Sinev, Jaydip Singh, J. Singh, L. Singh, P. Singh, V. Singh, S. Singh Chauhan, R. Sipos, C. Sironneau, G. Sirri, K. Siyeon, K. Skarpaas, J. Smedley, J. Smith, P. Smith, J. Smolik, M. Smy, M. Snape, E.L. Snider, P. Snopok, M. Soares Nunes, H. Sobel, M. Soderberg, H. Sogarwal, C. J. Solano Salinas, S. S\"oldner-Rembold, N. Solomey, V. Solovov, W. E. Sondheim, M. Sorbara, M. Sorel, J. Soto-Oton, A. Sousa, K. Soustruznik, D. Souza Correia, F. Spinella, J. Spitz, N. J. C. Spooner, D. Stalder, M. Stancari, L. Stanco, J. Steenis, R. Stein, H. M. Steiner, A. F. Steklain Lisb\^oa, J. Stewart, B. Stillwell, J. Stock, T. Stokes, T. Strauss, L. Strigari, A. Stuart, J. G. Suarez, J. Subash, A. Surdo, L. Suter, A. Sutton, K. Sutton, Y. Suvorov, R. Svoboda, S. K. Swain, C. Sweeney, B. Szczerbinska, A. M. Szelc, A. Sztuc, A. Taffara, N. Talukdar, J. Tamara, H. A. Tanaka, S. Tang, N. Taniuchi, A. M. Tapia Casanova, A. Tapper, S. Tariq, E. Tatar, R. Tayloe, A. M. Teklu, K. Tellez Giron Flores, J. Tena Vidal, P. Tennessen, M. Tenti, K. Terao, F. Terranova, G. Testera, T. Thakore, A. Thea, S. Thomas, A. Thompson, C. Thorpe, S. C. Timm, E. Tiras, V. Tishchenko, S. Tiwari, N. Todorovi{\'c}, L. Tomassetti, A. Tonazzo, D. Torbunov, D. Torres Mu{\~n}oz, M. Torti, M. Tortola, Y. Torun, N. Tosi, D. Totani, M. Toups, C. Touramanis, V. Trabattoni, D. Tran, J. Trevor, E. Triller, S. Trilov, D. Trotta, J. Truchon, D. Truncali, W. H. Trzaska, Y. Tsai, Y.-T. Tsai, Z. Tsamalaidze, K. V. Tsang, N. Tsverava, S. Z. Tu, S. Tufanli, C. Tunnell, M. Tuzi, M. Tzanov, M. A. Uchida, J. Ure{\~n}a Gonz{\'a}lez, J. Urheim, T. Usher, H. Utaegbulam, S. Uzunyan, M. R. Vagins, P. Vahle, G. A. Valdiviesso, E. Valencia, R. Valentim, Z. Vallari, E. Vallazza, J. W. F. Valle, R. Van Berg, D. V.  Forero, A. Vannozzi, M. Van Nuland-Troost, F. Varanini, D. Vargas Oliva, N. Vaughan, K. Vaziri, A. V{\'a}zquez-Ramos, J. Vega, J. Vences, S. Ventura, A. Verdugo, S. Vergani, M. Verzocchi, K. Vetter, M. Vicenzi, H. Vieira de Souza, C. Vignoli, C. Vilela, E. Villa, S. Viola, B. Viren, G. V. Stenico, R. Vizarreta, A. P. Vizcaya Hernandez, S. Vlachos, G. Vorobyev, Q. Vuong, A. V. Waldron, L. Walker, H. Wallace, M. Wallach, J. Walsh, T. Walton, L. Wan, B. Wang, H. Wang, J. Wang, M.H.L.S. Wang, X. Wang, Y. Wang, D. Warner, L. Warsame, M.O. Wascko, D. Waters, A. Watson, K. Wawrowska, A. Weber, C. M. Weber, M. Weber, H. Wei, A. Weinstein, S. Westerdale, M. Wetstein, K. Whalen, A.J. White, L. H. Whitehead, D. Whittington, F. Wieler, J. Wilhlemi, M. J. Wilking, A. Wilkinson, C. Wilkinson, F. Wilson, R. J. Wilson, P. Winter, J. Wolcott, J. Wolfs, T. Wongjirad, A. Wood, K. Wood, E. Worcester, M. Worcester, K. Wresilo, M. Wright, M. Wrobel, S. Wu, W. Wu, Z. Wu, M. Wurm, J. Wyenberg, B. M. Wynne, Y. Xiao, I. Xiotidis, B. Yaeggy, N. Yahlali, E. Yandel, G. Yang, J. Yang, T. Yang, A. Yankelevich, L. Yates, U. (. Yevarouskaya, K. Yonehara, T. Young, B. Yu, H. Yu, J. Yu, W. Yuan, M. Zabloudil, R. Zaki, J. Zalesak, L. Zambelli, B. Zamorano, A. Zani, O. Zapata, L. Zazueta, G. P. Zeller, J. Zennamo, J. Zettlemoyer, K. Zeug, C. Zhang, S. Zhang, Y. Zhang, L. Zhao, M. Zhao, E. D. Zimmerman, S. Zucchelli, V. Zutshi, R. Zwaska

